QUARK: A Framework for Quantum Computing Application Benchmarking

Quantum computing (QC) is anticipated to provide a speedup over classical HPC approaches for specific problems in optimization, simulation, and machine learning. With the advances in quantum computing toward practical applications, the need to analyze and compare different quantum solutions increases. While different low-level benchmarks for QC exist, these benchmarks do not provide sufficient insights into real-world application-level performance. We propose an application-centric benchmark method and the QUantum computing Application benchmaRK (QUARK) framework to foster the investigation and creation of application benchmarks for QC. This paper establishes three significant contributions: (1) it makes a case for application-level benchmarks and provides an in-depth "pen and paper" benchmark formulation of two reference problems: robot path and vehicle option optimization from the industrial domain; (2) it proposes the open-source QUARK framework for designing, implementing, executing, and analyzing benchmarks; (3) it provides multiple reference implementations for these two reference problems based on different known, and where needed, extended, classical and quantum algorithmic approaches and analyzes their performance on different types of infrastructures.

==> input_digitalewelt.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Input from Digitale Welt Article. 


\jknote{ The following is a copy paste from the article published in digitale welt. might be useful in terms of structure etc? See comment in .tex file for comments}

\begin{comment}
\emph{Robot Path Optimization}


%\alnote{Can we use a consistent vocabulary here: problem domain, problem class, mathematical formulation, algorithm?}




% \emph{QAOA:}
%The goal of solving any optimization problem is to find the best solution out of a set of many possible solutions. This can be interpreted as finding the ground state of a system which is defined by an energy or cost function. The Quantum Approximate Optimization Algorithm (QAOA)~\cite{farhi2014quantum} allows doing exactly that on gate-based Quantum computers. However, before starting to implement the algorithm, it is necessary to define a model of the real-world problem that needs to be solved. For instance, to verify that redundant components in a reusable spacecraft are never both working at the same time, can become a complex problem with an increasing number of components. However, it is crucial to perform this analysis, since such a design error could lead to a critical malfunction of the system. One approach to model this is by considering each component as a variable and the interactions and interdependencies between the components as SAT clauses. This results in a SAT problem with varying clause size. The constraints of the model depend on the restrictions of the real-world system. The mapping of the resulting problem to a quadratic binary optimization problem has been shown by [cite]. However, since gate-based Quantum computers allow to embed multi-body interactions, one can formulate a higher-order binary optimization problem. Each qubit is representing a variable of the problem. The interactions between the variables are represented by the weights of the  HOBO problem \alnote{HOBO not introduced} and are embedded through rotation and entangling gates between the respective set of qubits. If two qubits are not physically connected but the problem requires an interaction between the particular variables, one can use SWAP gates to bypass this challenge. However, this increases the length of the circuit and is therefore not an ideal solution for NISQ computers. After having formulated the problem, it can now be embedded in the QAOA procedure. (First, a Hadamard gate is applied to each qubit creating a uniform superposition state). After that, the problem is embedding through the entangling and Z rotation gates with an additional parameter $\gamma$. This step is called phase separation since the possible solutions of the optimization problem are separated by a phase factor $\gamma$. In the following, a so-called mixing Hamiltonian is applied that allows mapping the possible solution onto the computational basis state. Diverse circuits exist representing the Mixing Hamiltonian but usually contain X-rotation gates with a parameter value $\beta$. The measurement result of the final state is a Bit string corresponding to one possible component configuration. A classical computer now calculates the associated energy value. The goal is to use a classical optimizer which tries to find a set of parameters $\gamma$ and $\beta$ that minimize the energy value and therefore find an optimal solution to the initial problem.
%Overall, there is no silver bullet to develop a QAOA ansatz that solves every use-case optimally. Many parts of the algorithm need to be adapted to the problem. For instance, the mixing Hamiltonian can have a huge impact on the solution quality and aspects such as depth, expressibility, and the number of parameters need to be taken into consideration.
%An additional challenge is that when the circuit parameters are initialized randomly, the optimization procedure can get stuck at a so-called barren plateau. This describes an exponentially large plateau of states, for which the gradient between the objective values is very small. Therefore, finding an optimal set of parameters such that the optimal solution is found is highly unlikely. First solutions on how to mitigate this problem have been proposed but further investigation is necessary.
%}



%\jknote{Would  take this  out: As already mentioned, various problem classes exist within the automotive value chain. Many of the current algorithms to address those kind of problems do not show an exponential speed up over their classical counterparts \cite{algorithmzoo}. Nevertheless, the respective methods and algorithms are an active area of research while also allowing to investigate the applicability of Quantum Computing for real world Use-Cases. 
%One of that area addresses optimization problems. Broadly speaking optimization describes the process of finding the best solution out of a set of many possible solutions for one specific problem. They appear in almost every category of the BMW value chain. Therefore, finding good solutions for these problems is of high interest. Additionally, in the last few years, especially optimization problems where addressed by different Quantum Computing methods which can be implemented on NISQ devices. In the following, the approach on how this can be done for industry relevant problems and why they can work as benchmark problems is briefly explained.}
% \emph{Robot path optimization:}
\emph{Problem description:} In modern vehicle manufacturing, robots take on a significant workload, including performing welding jobs, sealing welding joints, or applying paint to the car body \cite{9108020}. While the robot's tasks vary widely, the objective remains the same: Perform a job with the highest possible quality in the shortest amount of time. %Since this is always connected to a certain path a robot needs to cover, the problem can be rephrased to: Perform the task by traveling the shortest path. 
For instance, to protect a car's underbody from corrosion, exposed welding seams are sealed by applying a polyvinyl chloride layer (PVC). The welding seams need to be traversed by a robot to apply the material. 


% The underlying mathematical model is the Traveling-Salesman-Problem (TSP) which is classified as NP-hard. 

\emph{Problem class and mathematical formulation:} The problem belongs to the domain of optimization problems, specifically to the class: traveling salesman problem, which is classified as NP-hard~\cite{TSP}. A typical mathematical formulation of the model is a weighted graph, which encodes the distance of all possible combinations of start- and endpoints. 
% Additionally, solutions in which not all seams have been processed or multiple seams need to be sealed simultaneously, are penalized. %by additional constraints.
The goal is to find a combination of connected start- and endpoints that represent the shortest path that needs to be traversed, and therefore, the shortest time necessary. A mathematical formulation suitable for a quantum computer is Quadratic Unconstrained Binary Optimization (QUBO), which can be derived from the traveling salesman graph~\cite{Lucas_2014}. We assign binary variables to the decision of assigning a robot to a specified seam at a discretized time, for all seams and all times.
Hence, for a problem with $N$ seams, $2 \times N^2$ variables are needed to model the connection between two points on the graph \cite{9108020}. %- taking into account that every seam can possibly be performed at every time step and all start and end points are connected \cite{9108020}. 

\emph{Algorithm:} The QUBO problem can then be solved using quantum annealing~\cite{DBLP:conf/kivs/MehtaMW17}. The most straightforward mapping requires $M$ qubits for $M$ binary variables. 
%\alnote{How many binary variable are on average required per seam?} 
%\jpnote{For N seams we need a total number of $2*N^2$ binary variables.} 
Another possible algorithm to solve this problem on a gate-based quantum computer is the Quantum Approximate Optimization Algorithm (QAOA) \cite{farhi2014quantum}. 

% In the resulting Hamiltonian equation, $Mathematical Equation needed$ quadratic terms are contained. 


%\jknote{at Josef: How many quadratic terms in the cost function? Then Each such term would in principle require a two-qubit entangling gate on a quantum computer? Can you recycle the entropica report: A: Formulation as QUBO, incl. info on required quadratic terms;  B: Embedding on Gate Based QC, incl. outlook in terms of scalabiliy; C: Annealing / Digital Annealing Solutions, incl. info on a} 

%The resulting binary vector permits to assign an address    


% It can be categorized as a hybrid algorithm since it embeds a problem on a gate-based Quantum Computer but also utilizes a classical computer to optimize parameters in the Quantum Circuit. 
% %The problem formulation as described above considers a set of interactions between two variables which represent the connection between two points on the graph. 
% %For a problem with $N$ seams, $2 \times N^2$ are needed to model the connection between two points on the graph %- taking into account that every seam can possibly be performed at every time step and all start and end points are connected \cite{9108020}. 

% The ground state of the Hamiltonian represents the optimal solution of the problem. In the QAOA ansatz, each variable is represented by a qubit. The $MathematiclEQUATION$ quadratic terms are embedded by two qubit entangling gates. For example, for a problem with $70$ Seams, $990$ two body terms are contained requiring twice as many entangling gates. However, since the error rate of those gates is currently very high, the outcome of the computation would not be usable. Therefore, to solve large scale TSP problems with a QAOA anasatz, a error corrected quantum computer would be needed. 

% In current Quantum Annealers, the two body interactions are directly embedded as a coupling strength between two qubits on the Hardware. They can therefore be understood as an analog computer which emulates an Ising system. These machines make use of the adiabatic theorem of Quantum mechanics. It roughly states that a system which is initially prepared in the groundstate will remain in this state as long as it changes slowly enough over time. To exploit this law, a Quantum Annealer tries to evolve from a trivial groundstate into a groundstate of the problem Hamiltonian by slowly changing the energy of the system. Ideally, the result is then an optimal solution of the described optimization problem. However, current Quantum Annealers such as provided by D-Wave suffer from analog control noise \cite{Pearson2019}. The result is that the probability of finding the optimal solution decreases exponentially with increasing problem size \cite{Albash2019}. 

% For nature inspired hardware such as the Fujitsu digital annealer, or Microsoft's QIO service noise is not the issue since these are classical technologies. However, with increasing problem size, the number of of constraints can exceed the number of variables. In such a case, it can already be computationally challenging to find a solution, that satisfies all the constraints. 


% %\todo[inline]{Josef: Entropica bericht einarbeiten (morgen)} 

% %\jknote{Entropica Report: However these operations are noisy, and at this scale the error rate would need to be around one part in a billion. This does not seem realistic without the use of quantum error correction, which in turn requires additional hardware overhead perhaps of the order of one thousand physical qubits per logical qubit. 
% %For quantum-inspired approaches such as Fujitsu's digital annealer, or Microsoft's QIO service, hardware limitations do not represent the main roadblock; after all, these are classical technologies. Instead, we encounter a scalability issue intrinsic to QUBO-encoded problems with certain types of constraint. The generic approach in re-formulating an optimisation problem as a QUBO involves adding any constraints as extra terms in the basic objective function. For example, in order to ensure we visit a seam with a valid address at each timeslot, we need to penalise solutions where this is not the case. As we make the problem size larger, the number of such constraint terms or clauses can outpace the number of variables itself. It then becomes very challenging for algorithms (including those at the heart of QIO technologies, such as parallel tempering, or simulated quantum annealing) to find any solution that even satisfies all the constraints, let alone one that minimises the energy or tour duration. For this reason, there tends to be a limit to the problem sizes that we can reliably solve in QUBO form}.



% \alnote{some remarks needed on what would constitute a reference problem based on PVC: dataset generator, reference implementation based on QUBO,....} \jknote{We have that above now,  correct?}

% %The interaction between any two variables is embedded by entangling and $Z$ rotation gates between the respective qubits. The angle of the rotation is given by the weight - in this problem distance - between the two variables. Additionally, a parameter $\gamma$ is added to the $Z$-rotation gates. This step of problem embedding and parameterizaton is called phase separation. This is due to the fact that all possible solutions of the optimization problem are separated by a phase factor $\gamma$ \cite{Phase_seperatoin}. Following, a mixing Hamiltonian is applied that is usually represented by a set of $X$-rotation gates and parameterized by an angle $\beta$. The mixing Hamiltonian allows to map a possible candidate solution onto the computational basis state \cite{hatfield}. Both steps, phase separation and mixing Hamiltonian are repeated with different parameters in each layer. The measurement outcome is a sequence of zeros and ones describing which seams are connected at what time step. By calculating the value of the cost function, a classical optimizer can adjust the parameter vectors $\vec{\gamma}$ and $\vec{\beta}$ such that the cost value is minimized \cite{farhi2014quantum}. 

%  %This QUBO formulation can also be embedded on special purpose Quantum machines such as the D-Wave Annealer or addressed with nature inspired algorithms such as simulated annealing. It therefore represents a possible benchmark problem which has both, high industry relevance due to various applications and a challenging complexity. 

% %\jknote{Josef, kannst du vielleicht grob vergleichen (qaoa vs annealing),  mit dem Ergebnis, dass man Industriereferenz Probleme braucht, um solche Fragen beantworten zu können?}

% %\jpnote{Klar, kann ich machen. Ich würde das nach dem Nessler (Extraaustattung) Use-Case machen, weil erst hier der unterschied zwischen Annealing und Gate based hervorsticht. (Argumentieren kann man dann das man verschiedene Industrie Use-Cases braucht um die verschiedenen Eigenschaften zu entdecken?) Der nächste Use-Case wäre um einiges kürzer, weil ja QAOA oben schon beschrieben wurde. }


\emph{Vehicle Configuration Optimization}
%\alnote{again: begin with problem statement - domain - class - formulation - solutions}

%The TSP is a good example of problems that can naturally be expressed in QUBO formulation. 

\emph{Problem description:} Newly developed car components need to be tested before moving into series production. For this purpose, test vehicles are built. This application's objective is to ensure that every new component is at least built into a test vehicle once. Since many different components are developed each year, the efficient allocation of components to test vehicles is essential, ensuring that the number of built test vehicles is minimal. A powerful engine requires a corresponding transmission. 

Further, there might be dependencies to other vehicle options, e.\,g., an interior design options might depend on the chosen engine. This example shows that the complex dependencies between components can result in a complex, combinatorial problem. Thus, minimizing the number of test vehicles can become highly complex. Similar, configuration problems arise in other areas, e.\,g., vehicle sequencing, optimizing vehicle configurations for built-to-stock vehicles, and in other industries, e.\,g., the production of other consumer goods.

%In many optimization problems, the interaction between variables is not restricted to be quadratic, turning them unsuitable for QUBO formulations. %For example, 
%The overall interconnectedness of the diverse components results in a challenging task to find valid combinations that contain as many newly developed parts as possible per vehicle. 
\emph{Problem class and mathematical formulation:}  This problem belongs to the class of boolean satisfiability problems (SAT). The different components are mapped to boolean variables, which are either $1$ (component is built in) or $0$ (component is not built in). Boolean clauses express the dependencies between the different components. The resulting mathematical formulation contains clauses with varying sizes, likely resulting in higher-order than quadratic terms (Polynomial Unconstrained Binary Optimization (PUBO)). %, turning them unsuitable for QUBO formulations.  

%Additional constraints such as that in each vehicle, two equipment items of the same type can not be build in allows restricting the solution space to the most relevant ones. 
%However, for clauses with many interacting components, a large overhead of additional variables is generated. %For example, in a boolean term with 5 components, all 5 variables are interconnected. 

\emph{Algorithm:} Even though it has been shown that SAT problems can also be mapped to QUBO problems, the reformulation of higher-order terms as quadratic functions leads to a high amount of ancillary variables. To avoid this increase of variables, the QAOA can, e.\,g., be used to solve the resulting PUBO problem \cite{Hadfield2018}. 



% Gate-based Quantum Computers allow to embed multibody interactions directly. Finding an optimal solution for the resulting Hamiltonian can therefore be mathematically formulated as a Polynomial Unconstrained Binary Optimization (PUBO) problem. The contained mutibody interactions are embedded through entangling the respective qubits. Thereby, $N$ components can be represented by $N$ qubits. 
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
